Characterizing SLAM Benchmarks and Methods for the Robust Perception Age

The diversity of SLAM benchmarks affords extensive testing of SLAM algorithms to understand their performance, individually or in relative terms. The ad-hoc creation of these benchmarks does not necessarily illuminate the particular weak points of a SLAM algorithm when performance is evaluated. In this paper, we propose to use a decision tree to identify challenging benchmark properties for state-of-the-art SLAM algorithms and important components within the SLAM pipeline regarding their ability to handle these challenges. Establishing what factors of a particular sequence lead to track failure or degradation relative to these characteristics is important if we are to arrive at a strong understanding for the core computational needs of a robust SLAM algorithm. Likewise, we argue that it is important to profile the computational performance of the individual SLAM components for use when benchmarking. In particular, we advocate the use of time-dilation during ROS bag playback, or what we refer to as slo-mo playback. Using slo-mo to benchmark SLAM instantiations can provide clues to how SLAM implementations should be improved at the computational component level. Three prevalent VO/SLAM algorithms and two low-latency algorithms of our own are tested on selected typical sequences, which are generated from benchmark characterization, to further demonstrate the benefits achieved from computationally efficient components.

==> bigtable.tex <==
\newpage
\begin{sidewaystable*}
\caption{Summary of VSLAM datasets}
\label{tab:summ_vslam}
\centering
\begin{threeparttable}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
	\toprule[1.5pt]
	\multirow{2}{*}{\bfseries Dataset} & \multirow{2}{*}{\bfseries Year} & \multirow{2}{*}{\bfseries Environ.} & \bfseries Environ. & \multirow{2}{*}{\bfseries Platform}
	& \bfseries Motion & \bfseries Motion & \multirow{2}{*}{\bfseries Duration\tnote{3}} 
	& \bfseries Revisit & \bfseries Multi- & \multicolumn{3}{c|}{\bfseries Sensor Setting} & \bfseries Ground\\
	\cline{11-13}
	& & & \bfseries Dynamics\tnote{1} & & \bfseries Profile & \bfseries Dynamics\tnote{2} & & \bfseries Freq.\tnote{4} & \bfseries Sesson &	 \bfseries Stereo\tnote{5} & \bfseries IMU & \bfseries Lidar & \bfseries Truth \\ 
	\midrule[1.5pt]
	NewCollege\cite{smith2009new} 		& 2009 & outdoor & D & Segway & 6 DoF & SS+SA & LT & HF & F & \cmark & \cmark & \xmark & \xmark \\
	Rawseeds\cite{fontana2014rawseeds} 	& 2009 & in-/outdoor & D & Ground Robot & 2 DoF &  &  & MF & F & \cmark & \cmark & \cmark & \cmark \\
	MIT DARPA\cite{huang2010high} 		& 2010 & & & & & & & & & & \cmark & \cmark & \cmark \\
	The Marulan\cite{peynot2010marulan} & 2010 & & & & & & & & & \xmark  & \cmark & \cmark  & \cmark \\
	Karlsruhe\cite{Geiger2010ACCV} 		& 2010 & & & & & & & & & \cmark  & \cmark   &\xmark   & \cmark \\
	Ford Campus\cite{pandey2011ford} 	& 2011 & outdoor & HD & Truck & 2 DoF & FS+SA & MT & MF & F & \cmark & \cmark & \cmark & \xmark \\
	CMU-VL\cite{badino2011visual} 		& 2011 & outdoor & HD & Car & 2 DoF & FS+SA & LT &  HF & T  & \cmark &  & \xmark & \xmark \\
	TUM RGBD\cite{sturm12iros} 			& 2012 & indoor & D & Handheld\! \&\! Pioneer & 2/3 DoF & & ST & LF & F  & \cmark & \cmark & Depth & \\
	KITTI\cite{KITTI} 					& 2013 & outdoor & HD & Car & 2 DoF & FS+SA & ST & LF & F  & \cmark & \cmark & \cmark & \xmark \\
	Malaga Urban\cite{blanco2014malaga} & 2014 & outdoor & HD & Car & 2 DoF & & & HF & F  & \cmark & \cmark & \cmark & \xmark \\
	ICL NUIM\cite{ICLNUIM} 				& 2014 & indoor & S & Handheld & 6 DoF & &  & LF & F  & \cmark &  & Depth & \cmark \\
	UMich NCLT\cite{carlevaris2016university} & 2015 & in-/outdoor & HD & Segway & 2 DoF & & & HF & T & \cmark & \cmark & \cmark & \\
	EuRoC\cite{burri2016euroc} 			& 2016 & indoor & LD & MAV & 6 DoF & All & ST & MF & F  & \cmark & \cmark & \xmark & \cmark \\
	TUM Mono\cite{engel2016monodataset} & 2016 & in-/outdoor & LD & Handheld & 6 DoF & & ST & LF & F  & \xmark & \xmark & \xmark & \\
	PennCOSYVIO\cite{pfrommer2017penncosyvio} & 2017 & in-/outdoor & LD & Handheld & 3 DoF & &  & MF & F  & \cmark & \cmark & \xmark & \\
	Zurich Urban MAV\cite{majdik2017zurich} & 2017 & outdoor &  & MAV & 6 DoF & & ST & LF & F  & \cmark & \cmark & \xmark & \\
	RobotCar\cite{maddern20171} 			& 2017 & outdoor & HD & Car & 2 DoF &  & LT & HF & T  & \cmark & \cmark & \cmark & \\
	TUM VI\cite{schubert2018vidataset}	 	& 2018 & in-/outdoor &  & Handheld & 3 DoF &  & ST &  & F  & \cmark & \cmark & \cmark & \\
	Interior Net\cite{li2018interiornet} 	& 2018 & indoor & LD & Simulated & 6 DoF &  &  &  & T  & \cmark & \cmark & Depth & \cmark\\
	BlackBird\cite{antonini2018blackbird} 	& 2018 & indoor & LD & MAV & 6 DoF &  &  &  & F  & \cmark & \cmark & \xmark & \cmark\\
	UZH-FPV\cite{delmericowe} 				& 2019 & in-/outdoor & S & MAV & 6 DoF & FS+FA &  &  & T  & \cmark & \cmark & \xmark & \cmark\\
	\bottomrule[1.5pt]
\end{tabular}
      \begin{tablenotes}
        \footnotesize
        \item[1]	Environ. Dynamics: Static(S), Low Dynamic(LD), Dynamic(D), High Dynamic(HD);
        \item[2]	Motion Dynamics: Slow Smooth(SS), Slow Aggressive(SA), Fast Smooth(FS), Fast Aggressive(FA);
		\item[3]	Duration: Short Term(ST), Mid Term(MT), Long Term(LT);
		\item[4]	Revisit Freq.: Low Frequency(LF), Medium Frequency(MF), High Frequency(HF);
   		\item[5]	"Stereo" contains sensor settings with at lease two optical cameras
      \end{tablenotes}
      \end{threeparttable}
\end{sidewaystable*}
\clearpage




==> tabaccuracy.tex <==
\begin{table*}[t]
	\small
	\centering
	\caption{RMSE (M) / RPE (M/S) of 3 VO algorithms in slo-mo/normal speed on Selected Sequences}
	\begin{tabular}{c|c||c|c|c||c|c|c|c|c}
		\toprule[1pt]
		\midrule[0.1pt]
		\textbf{ } & 
		& \multicolumn{3}{c||}{\bfseries \small one run in \textit{slo-mo}}
		& \multicolumn{5}{c}{\bfseries \small five runs in normal speed (\#failures are highlighted by -/\textcolor{f4}{4}/\textcolor{f3}{3}/\textcolor{f2}{2}/\textcolor{f1}{1}/0)} \\
		\cmidrule{3-10}
		& \textbf{\small Seq.} & SVO\cite{SVO2017} & DSO\cite{DSO2017} & ORB\cite{ORBSLAM}  & SVO\cite{SVO2017} & DSO\cite{DSO2017} & ORB\cite{ORBSLAM} & GoodFeature\cite{zhao2018good2} & MapHash\cite{zhao2019maphash} \\
		\midrule
		\  \parbox[t]{1mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{RMSE}}}} \ 
				
		& \textit{f2 desk person}  & 1.26e0 	& 1.25e-1	& \underline{4.76e-2}  & \textcolor{f1}{1.53e0}& \textcolor{f0}{5.36e-1}& \textcolor{f0}{5.94e-2} & \textcolor{f0}{3.51e-2} &  \underline{\textcolor{f0}{2.88e-2}}\\
		
		& \textit{lr kt0}			& 4.97e-1	& 2.21e-1	&	\underline{2.10e-1}	 & \textcolor{f0}{3.07e-1} & \underline{\textcolor{f0}{2.61e-1}} & - & - & -			\\		
		
		& \textit{of kt3}			& 6.43e-1	& \underline{3.82e-2}	&	5.58e-2		 &\textcolor{f0}{5.60e-1} & \underline{\textcolor{f0}{3.87e-2}}&\textcolor{f0}{2.57e-1} & \textcolor{f0}{2.76e-1} & 	 \textcolor{f0}{6.69e-2}	\\
		
		& \textit{room3}  			& 2.03e0	& 2.86-1	& \underline{2.09e-1}  & \textcolor{f2}{2.02e0}& - & \underline{\textcolor{f2}{1.80e-1}} & -&  -\\ 		
		
		& \textit{outdoors4}  		& -		 	& \underline{2.21e-2} 	& 8.39e-2  & \underline{\textcolor{f3}{1.74e0}}& - & - & -&  -\\ 
				
		& \textit{MH 05 diff}  		& 4.26e0 	& \underline{1.38e-1}	& 3.03e-1 &  \textcolor{f1}{1.44e0} & \underline{\textcolor{f4}{1.08e-1}}& \textcolor{f0}{1.18e0} & \textcolor{f0}{1.43e-1} & \textcolor{f0}{2.29e-1}\\ 
		
		& \textit{V1 01 diff}  		& 5.53e-1 	& 1.08e0 	& \underline{2.32e-1}  & \textcolor{f0}{6.09e-1} & \textcolor{f0}{1.34e0}& \textcolor{f3}{1.25e0}& \textcolor{f4}{9.23e-1}&  \underline{\textcolor{f2}{4.61e-1}}\\ 
		
		%
		\midrule
		\  \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{RPE}}}}\ 
				
		& \textit{KITTI Seq 04} 	& 2.06e0 	& \underline{7.88e-2} 	& 9.18e-2  & \textcolor{f0}{1.82e0} & \underline{\textcolor{f0}{8.09e-2}}&\textcolor{f0}{9.74e-2} & \textcolor{f0}{1.00e-1} &  \textcolor{f0}{9.92e-2} \\ 
		
		& \textit{KITTI Seq 02}		& 6.91e0		& \underline{1.31e-1}		& 1.38e-1	 & \textcolor{f0}{7.17e0} & \textcolor{f0}{1.52e-1}& \textcolor{f2}{2.08e-1} & - &  \underline{\textcolor{f3}{1.41e-1}}\\	
		
		& \textit{conf. hall1} 		& 4.35e-1  & \underline{4.33e-1}	& -	 & \textcolor{f0}{4.25e-1}& \textcolor{f0}{4.57e-1}& \underline{\textcolor{f4}{1.50e-1}}& \textcolor{f0}{1.64e-1}& \textcolor{f1}{2.17e-1}\\%\textbf{2.24e-1} \\ 
		
		& \textit{corridor}			& 1.20e0	&	6.50e-1		&	\underline{2.34e-1}	 & \textcolor{f0}{1.38e0}& \underline{\textcolor{f0}{5.31e-1}}& \textcolor{f4}{1.54e0}& \textcolor{f0}{6.22e-1}& \textcolor{f1}{1.05e0}\\
		
		& \textit{NewCollege}  		& -        & 1.92e-2   & \underline{1.65e-2}  & - & \textcolor{f0}{1.93e-2} & \underline{\textcolor{f1}{1.88e-2}}& \textcolor{f0}{1.95e-2}&  \textcolor{f0}{1.92e-2}\\ 	
		\midrule[0.1pt]
 	\bottomrule	[1pt]
	\end{tabular} 
	\label{tab:accuracy_summary}
\end{table*}
